FP8 Quantization: The Power of the Exponent

When quantizing neural networks for efficient inference, low-bit integers are the go-to format for efficiency. However, low-bit floating point numbers have an extra degree of freedom, assigning some bits to work on an exponential scale instead. This paper in-depth investigates this benefit of the floating point format for neural network inference. We detail the choices that can be made for the FP8 format, including the important choice of the number of bits for the mantissa and exponent, and show analytically in which settings these choices give better performance. Then we show how these findings translate to real networks, provide an efficient implementation for FP8 simulation, and a new algorithm that enables the learning of both the scale parameters and the number of exponent bits in the FP8 format. Our chief conclusion is that when doing post-training quantization for a wide range of networks, the FP8 format is better than INT8 in terms of accuracy, and the choice of the number of exponent bits is driven by the severity of outliers in the network. We also conduct experiments with quantization-aware training where the difference in formats disappears as the network is trained to reduce the effect of outliers.

==> checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{To the best of our knowledge, efficient representations for neural network do not have any negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical claims.}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical claims.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{All models and data is publicly available, the code of our FP8 simulation is proprietary.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See section~\ref{sec:baselines} and supplementary material.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Most results are deterministic and only depend on the pre-trained model (with exception of QAT results in Table~\ref{tab:qat}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See section~\ref{sec:baselines}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> tables/bert_fp8_ptq_tables.tex <==
\begin{table}[h]

    \begin{subtable}[]{\textwidth}
        \begin{tabular}{ll|llllllll|l}
        Mantissa bits & Bias & CoLA  & SST-2 & MRPC  & STS-B  & QQP   & MNLI  & QNLI  & RTE   & Macro avg \\
        \hline
        FP32          &      & 57.27 & 93.12 & 88.36 & 89.09  & 89.72 & 84.91 & 91.58 & 70.40 & 83.06     \\
        
        4             & 1    & -6.26 & 75.46 & 27.19 & -10.63 & 60.77 & 48.52 & 51.36 & 48.74 & 36.89     \\
                      & 2    & 47.92 & 90.83 & 84.05 & 86.60  & 86.86 & 80.30 & 85.87 & 66.79 & 78.65     \\
                      & 3    & 11.42 & 86.24 & 74.10 & 67.76  & 55.31 & 65.61 & 75.38 & 59.57 & 61.92     \\
                      & 4    & 1.53  & 84.17 & 74.33 & 34.66  & 64.97 & 41.81 & 53.10 & 57.04 & 51.99     \\
        3             & 7    & 57.53 & 92.89 & 87.55 & 88.90  & 89.77 & 84.84 & 91.34 & 68.95 & 82.72     \\
                      & 8    & 57.31 & 92.78 & 87.96 & 89.03  & 89.73 & 84.71 & 91.51 & 69.68 & 82.84     \\
                      & 9    & 56.51 & 92.32 & 88.16 & 88.99  & 89.79 & 84.87 & 91.69 & 68.59 & \textbf{83.06}    
        \end{tabular}
        \caption{Results on BERT for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    \end{subtable}
    
    \begin{subtable}[]{\textwidth}
        \begin{tabular}{ll|llllllll|l}
        Mantissa bits & Bias & CoLA  & SST-2 & MRPC  & STS-B & QQP   & MNLI  & QNLI  & RTE   & Macro avg\\
                           \hline
        4 & Flexible & 56.51 & 92.32 & 88.16 & 88.99 & 89.79 & 84.87 & 91.69 & 68.59 & 82.61             \\
        3 & Flexible & 57.29 & 93.12 & 87.35 & 88.87 & 89.76 & 84.87 & 91.51 & 69.68 & \textbf{82.80}              \\
        \end{tabular}
        \caption{Results on BERT for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    \end{subtable}
    
    
    \begin{subtable}[]{\textwidth}
        \begin{tabular}{l|llllllll|l}
                       & CoLA  & SST-2 & MRPC  & STS-B & QQP   & MNLI  & QNLI  & RTE   & Macro avg ex. WNLI \\
        \hline
        Fully flexible & 57.78 & 93.00 & 88.57 & 89.04 & 89.77 & 84.86 & 91.41 & 69.68 & 83.02             
        \end{tabular}
        \caption{Results on BERT for fully flexible FP8 formats. Mantissa and exponent bits are set individually per quantizer, bias is set per channel.}
    \end{subtable}
    \caption{BERT PTQ results}\label{tab:bertfull}
\end{table}

==> tables/dlv3_fp8_ptq_tables.tex <==
\begin{table}[]
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN &  Reest BN & Original BN &  Reest BN \\
        Mantissa bits & Bias &             &           &             &           \\
        \hline
        5 & -2  &    3.268 &  3.268 &    3.268 &  3.268 \\
          & -1  &    3.268 &  3.268 &    3.268 &  3.268 \\
          &  0  &    3.268 &  3.268 &    3.268 &  3.268 \\
          &  1  &    3.268 &  3.268 &    3.268 &  3.268 \\
        4 &  2  &    3.268 &  3.268 &    3.268 &  3.268 \\
          &  3  &    3.268 &  3.268 &    3.268 &  3.268 \\
          &  4  &    3.268 &  3.268 &    3.268 &  3.268 \\
          &  5  &    3.268 &  3.268 &    3.268 &  3.268 \\
        3 &  8  &    \textbf{9.423} &  \textbf{9.423} &    \textbf{9.423} &  \textbf{9.423} \\
          &  9  &    9.122 &  9.122 &    9.122 &  9.122 \\
          &  10 &    8.893 &  8.893 &    8.893 &  8.893 \\
          &  11 &    3.268 &  3.268 &    3.268 &  3.268 \\
        \end{tabular}
        \caption{Results on DeepLabV3 for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    \end{subtable}

    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN &   Reest BN & Original BN &   Reest BN \\
        Exponent bits & Range setting &             &            &             &            \\
        \hline
        5 & MSE, MSE &   \textbf{72.579} &  \textbf{72.579} &   62.318 &  62.318 \\
          & current\_minmax, allminmax &   71.672 &  71.672 &   63.859 &  63.859 \\
          & current\_minmax, running\_minmax &   71.672 &  71.672 &   63.859 &  63.859 \\
        4 & MSE, MSE &   71.283 &  71.283 &   35.428 &  35.428 \\
          & current\_minmax, allminmax &   62.216 &  62.216 &   51.547 &  51.547 \\
          & current\_minmax, running\_minmax &   62.216 &  62.216 &   51.547 &  51.547 \\
        3 & MSE, MSE &   37.930 &  37.930 &   12.949 &  12.949 \\
          & current\_minmax, allminmax &   22.143 &  22.143 &   21.951 &  21.951 \\
          & current\_minmax, running\_minmax &   22.143 &  22.143 &   21.951 &  21.951 \\
        \end{tabular}
        \caption{Results on DeepLabV3 for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    \end{subtable}

    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{l|rrrr}
         & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
         & Original BN &   Reest BN & Original BN &   Reest BN \\
        Range setting &             &            &             &            \\
        \hline
        MSE, MSE      &   \textbf{72.722} &  \textbf{72.722} &   63.043 &  63.043 \\
        \end{tabular}
        \caption{Results on DeepLabV3 for fully flexible FP8 formats. Mantissa and exponent bits are set individually per quantizer, bias is set per channel. Best results are marked in bold.}
    \end{subtable}
    \caption{DeepLabV3 PTQ results}\label{tab:dlv3full}

\end{table}

==> tables/hrnet_fp8_ptq_tables.tex <==
\begin{table}[h!]
    \begin{subtable}[]{\textwidth}
    % \begin{subfloat}[Results on SalsaNext for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.]
        \centering
        \begin{tabular}{ll|r}
        Mantissa bits & Bias & mIoU \\
        \hline
        3 &  8  & 80.71 \\
        4 &  4  & 0.48 \\
        \end{tabular}
        \caption{Results on HRNet for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    % \end{subfloat}
    \end{subtable}
    
    
    \begin{subtable}[]{\textwidth}
    % \begin{subfloat}[Results on SalsaNext  esm  ,÷ for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.]
        \centering
        \begin{tabular}{ll|r}
         Mantissa bits & Range setting & MIoU \\
        \hline
        5 & MSE, MSE &      81.03  \\
        4 & MSE, MSE &      81.04  \\
        3 & MSE, MSE &      80.77  \\
        \end{tabular}
        \caption{Results on HRNet for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    % \end{subfloat}
    \end{subtable}
    \caption{HRNet PTQ results}\label{tab:hrnetfull}
\end{table}

==> tables/mnv2_fp8_ptq_tables.tex <==
\begin{table}
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
        
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Bias &             &          &             &          \\
        \hline
        5 & -2  &       0.100 &    0.100 &       0.100 &    0.100 \\
          & -1  &       0.100 &    0.102 &       0.100 &    0.102 \\
          &  0  &       0.110 &   20.352 &       0.110 &   20.352 \\
          &  1  &       5.578 &   15.212 &       5.578 &   15.212 \\
        4 &  2  &      20.630 &   62.950 &      20.630 &   62.950 \\
          &  3  &      53.762 &   \textbf{68.490} &      53.762 &   \textbf{68.490} \\
          &  4  &      57.256 &   60.420 &      57.256 &   60.420 \\
          &  5  &       7.538 &    6.440 &       7.538 &    6.440 \\
        3 &  8  &      50.990 &   66.496 &      50.990 &   66.496 \\
          &  9  &      50.912 &   66.234 &      50.912 &   66.234 \\
          &  10 &      50.968 &   66.386 &      50.968 &   66.386 \\
          &  11 &      50.976 &   66.362 &      50.976 &   66.362 \\
        
        \end{tabular}
        \caption{Results on MobileNetV2 for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    \end{subtable}
        
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
        
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Range setting &             &          &             &          \\
        \hline
        5 & MSE, MSE &      70.052 &   70.116 &      63.102 &   68.106 \\
          & current\_minmax, allminmax &      70.300 &   \textbf{71.058} &      63.012 &   71.046 \\
          & current\_minmax, running\_minmax &      70.300 &   \textbf{71.058} &      63.012 &   71.046 \\
        4 & MSE, MSE &      68.820 &   70.586 &      66.980 &   70.620 \\
          & current\_minmax, allminmax &      67.190 &   70.008 &      65.676 &   70.024 \\
          & current\_minmax, running\_minmax &      67.190 &   70.008 &      65.676 &   70.024 \\
        3 & MSE, MSE &      52.312 &   64.658 &      52.794 &   64.532 \\
          & current\_minmax, allminmax &      55.076 &   64.430 &      47.646 &   66.050 \\
          & current\_minmax, running\_minmax &      55.076 &   64.430 &      47.646 &   66.050 \\
        
        \end{tabular}
        \caption{Results on MobileNetV2 for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    \end{subtable}
        
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{l|rrrr}
        
         & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
         & Original BN & Reest BN & Original BN & Reest BN \\
        Range setting &             &          &             &          \\
        \hline
        MSE, MSE      &       70.13 &   \textbf{71.284} &        66.5 &   71.206 \\
        
        \end{tabular}
        \caption{Results on MobileNetV2 for fully flexible FP8 formats. Mantissa and exponent bits are set individually per quantizer, bias is set per channel. Best results are marked in bold.}
    \end{subtable}
    \caption{MobileNetV2 PTQ results}\label{tab:mnv2full}

\end{table}

==> tables/ptq1.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|r r|r r r}
        Model & FP32 & INT8 & 1/4/3/8 & 1/3/4/4 & 1/2/5/2 \\
        \hline
         ResNet18 &  \multirow{2}{*}{69.72\%} & 69.29\% & 68.13\% & 58.72\% & 0.13\% \\
         ResNet18 (+BN re-est) & & \textbf{69.54\%} & 68.49\% & 61.01\% & 0.49 \% \\
         \hline
         MobileNetV2 & \multirow{2}{*}{71.70\%} & 0.08\% & 43.49\% & 39.35\% & \\
         MobileNetV2 (+BN re-est) & & \textbf{67.06\%} & 66.26\% & 60.12\% & \\
         \hline
         BERT (GLUE macro avg) & 83.06\% & 71.03\% & \textbf{82.84\%} & 51.99\% & \\
         \hline
         SalsaNext (SemanticKITTI) & 0.558 & 0.530 & 0.549 & \textbf{0.554}
    \end{tabular}
    \caption{PTQ results with standard FP8 formats. Results in boldface indicate the best PTQ results for each model.}
    \label{tab:ptq1}
\end{table}

==> tables/ptq2.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{l|r r|r r r r r r}
%         Model                       & FP32                      & INT8              & 1/4/3/8   & 1/4/3/9   & 1/3/4/4           & 1/3/4/3 & 1/2/5/2 & 1/2/5/-1 \\
%         \hline
%          ResNet18                   &  \multirow{2}{*}{69.72} & 69.29           & 68.13   & 68.22   & 58.72           & 54.80 &  0.13  & 0.99\\
%          ResNet18 (+BN re-est)
%          &                      & \textbf{69.54}  & 68.49   & 68.52   & 61.01           & 68.45 & 0.49  & 27.43 \\
%          \hline
%          MobileNetV2                & \multirow{2}{*}{71.70}  & 0.08 & 43.49  & 43.51   & 39.35   & 36.26           & \\
%          MobileNetV2 (+BN re-est)   
%          &      & 67.06 & 66.26 & 66.41   & 60.12   & \textbf{68.32}  & \\
%          \hline
%          SalsaNext  & 0.558                     & 0.530             & 0.549     & 0.549     & \textbf{0.554}    &
%     \end{tabular}
%     \caption{PTQ results with standard FP8 formats. Results in boldface indicate the best PTQ results for each model. We compare non-standard bias values to the standard bias value for each exponent/mantissa division.}
%     \label{tab:ptq2}
% \end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{l|r r|r r r r r r}
%         Model                       & FP32                      & INT8              & 1/4/3/8   & 1/4/3/9   & 1/3/4/4           & 1/3/4/3 & 1/2/5/2 & 1/2/5/-1 \\
%         \hline
%         ResNet18$\dagger$    &  69.72                     & \textbf{69.54}  & 68.49   & 68.52   & 61.01           & 68.45 & 0.49  & 27.43 \\
%         MobileNetV2$\dagger$   &         71.70      & 67.06 & 66.26 & 66.41   & 60.12   & \textbf{68.32}  & \\
%          SalsaNext  & 0.558                     & 0.530             & 0.549     & 0.549     & \textbf{0.554}    &
%     \end{tabular}
%     \caption{PTQ results with standard FP8 formats. Results in boldface indicate the best PTQ results for each model. We compare non-standard bias values to the standard bias value for each exponent/mantissa division.}
%     \label{tab:ptq2}
% \end{table}

\begin{table}[]
    \centering
    \begin{tabular}{l|r r|r r r r}
        Model                       & FP32                      & INT8              & 3M4E8B   & 3M4E9B  & 4M3E4B           & 4M3E3B \\
        \hline
        ResNet18    &  69.72                     & 69.54  & 68.49   & 68.52   &  61.01           & 68.45 \\
        MobileNetV2   &         71.70      & 67.06 & 66.26 & 66.41     & 60.12   & 68.32         \\
        SalsaNext  & 55.80  & 53.02            & 54.90     & 54.89        & 55.40    & 55.79
    \end{tabular}
    \caption{PTQ results with standard FP8 formats. Results in boldface indicate the best PTQ results for each model. We compare non-standard bias values to the standard bias value for each exponent/mantissa division.}
    \label{tab:ptq2}
\end{table}

==> tables/ptq3.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{l|r r|r r r r r r}
%         Model                       & FP32                      & INT8      & 1/4/3/9   & 1/4/3/*   & 1/3/4/3   & 1/3/4/*   & 1/2/5/* \\
%         \hline
%          ResNet18                   & \multirow{2}{*}{69.72\%}  & 69.29\%   & 68.22\%   & 67.92\%   & 54.80\%   & 69.27\%   & 69.46\% \\
%          ResNet18 (+BN re-est)      &                           & \textbf{69.54\%}   & 68.52\%   & 68.39\%   & 68.45\%   & \textbf{69.54\%}   & 69.51\% \\
%          \hline
%          MobileNetV2                & \multirow{2}{*}{71.70\%}  & 0.08\%    & 43.51\%   & 43.46\%   & 36.26\%   & 50.98\%   & 0.10\%  \\
%          MobileNetV2 (+BN re-est)   &                           & 67.06\%   & 66.41\%   & 66.36\%   & 68.32\%   & 69.80\%   & \textbf{71.19\%} \\
%          \hline
%          BERT (GLUE macro avg)      & 83.06\%                   & 71.03\%   & \textbf{82.84\%}   & 82.80\%     & 61.92\%   & 82.61\%   & \\
%     \end{tabular}
%     \caption{PTQ results with flexible bias. Results in boldface indicate the best PTQ results for each model. We compare flexible bias values to the best fixed bias value for each exponent/mantissa division.}
%     \label{tab:ptq3}
% \end{table}


\begin{table}[]
    \centering
    \begin{tabular}{l|r r|r r r r r r}
        Model                       & FP32                      & INT8      & 1/4/3/9   & 1/4/3/*   & 1/3/4/3   & 1/3/4/*   & 1/2/5/* \\
        \hline
         ResNet18 $\dagger$ &   69.72\%    & \textbf{69.54\%}   & 68.52\%   & 68.39\%   & 68.45\%   & \textbf{69.54\%}   & 69.51\% \\
         MobileNetV2 $\dagger$   &  71.70\% & 67.06\%   & 66.41\%   & 66.36\%   & 68.32\%   & 69.80\%   & \textbf{71.19\%} \\
         BERT & 83.06\%                   & 71.03\%   & \textbf{82.84\%}   & 82.80\%     & 61.92\%   & 82.61\%   & \\
    \end{tabular}
    \caption{PTQ results with flexible bias. Results in boldface indicate the best PTQ results for each model. We compare flexible bias values to the best fixed bias value for each exponent/mantissa division.}
    \label{tab:ptq3}
\end{table}

==> tables/ptq4.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{l|r r|r r r r r r}
%         Model                       & FP32                      & INT8      && 1/4/3/*   && 1/3/4/*   & 1/2/5/*     & 1/*/*/* \\
%         \hline
%          ResNet18                   & \multirow{2}{*}{69.72\%}  & 69.29\%   && 67.92\%   && 69.27\%   & 69.46\%     & 69.40\% \\
%          ResNet18 (+BN re-est)      &                           &69.54\%    && 68.39\%   && 69.54\%   & 69.51\%     & \textbf{69.63\%} \\
%          \hline
%          MobileNetV2                & \multirow{2}{*}{71.70\%}  & 0.08\%    && 43.46\%   && 50.98\%   & 0.10\%      & 40.74\% \\
%          MobileNetV2 (+BN re-est)   &                           & 67.06\%   && 66.36\%   && 69.80\%   & \textbf{71.19\%}     & 71.08\% \\
%          \hline
%          BERT (GLUE macro avg)      & 83.06\%                   & 71.03\%   && 82.80\%   && 82.61\%   &             & \textbf{83.02\%} \\
%     \end{tabular}
%     \caption{PTQ results with flexible bias and fully flexible FP8 formats. Results in boldface indicate the best PTQ results for each model.}
%     \label{tab:ptq4}
% \end{table}



\begin{table}[]
    \centering
    \begin{tabular}{l|r r|r r r r r r}
        Model                       & FP32                      & INT8      && 1/4/3/*   && 1/3/4/*   & 1/2/5/*     & 1/*/*/* \\
        \hline
         ResNet18 $\dagger$      &  69.72\%  &69.54\%    && 68.39\%   && 69.54\%   & 69.51\%     & \textbf{69.63\%} \\
         MobileNetV2 $\dagger$ &  71.70\% & 67.06\%   && 66.36\%   && 69.80\%   & \textbf{71.19\%}     & 71.08\% \\
         BERT  & 83.06\%                   & 71.03\%   && 82.80\%   && 82.61\%   &             & \textbf{83.02\%} \\
    \end{tabular}
    \caption{PTQ results with flexible bias and fully flexible FP8 formats. Results in boldface indicate the best PTQ results for each model.}
    \label{tab:ptq4}
\end{table}

==> tables/rn18_fp8_ptq_tables.tex <==
\begin{table}[h!]
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Bias &             &          &             &          \\
        \hline
        5 & -2  &       0.100 &    0.136 &       0.100 &    0.136 \\
          & -1  &       0.100 &    0.512 &       0.100 &    0.512 \\
          &  0  &       0.220 &   21.096 &       0.220 &   21.096 \\
          &  1  &      15.112 &   27.248 &      15.112 &   27.248 \\
        4 &  2  &      51.546 &   63.580 &      51.546 &   63.580 \\
          &  3  &      66.510 &   68.346 &      66.510 &   68.346 \\
          &  4  &      59.090 &   60.862 &      59.090 &   60.820 \\
          &  5  &       8.232 &    8.464 &       8.232 &    8.480 \\
        3 &  8  &      68.220 &   68.440 &      68.220 &   68.440 \\
          &  9  &      68.126 &   \textbf{68.521} &      68.126 &   68.428 \\
      &  10 &      68.228 &   68.442 &      68.228 &   68.440 \\
          &  11 &      68.126 &   68.380 &      68.126 &   68.380 \\
        \end{tabular}
        \caption{Results on ResNet18 for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    \end{subtable}

    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Range setting &             &          &             &          \\
        \hline
        5 & MSE, MSE &      69.470 &   69.566 &      69.374 &   69.548 \\
          & current\_minmax, allminmax &      69.492 &   69.632 &      69.514 &   \textbf{69.658} \\
          & current\_minmax, running\_minmax &      69.486 &   69.632 &      69.514 &   \textbf{69.658} \\
        4 & MSE, MSE &      69.186 &   69.284 &      69.294 &   69.368 \\
          & current\_minmax, allminmax &      69.110 &   69.424 &      69.288 &   69.434 \\
          & current\_minmax, running\_minmax &      69.110 &   69.424 &      69.276 &   69.450 \\
        3 & MSE, MSE &      68.212 &   68.570 &      67.976 &   68.392 \\
          & current\_minmax, allminmax &      68.110 &   68.230 &      68.030 &   68.292 \\
          & current\_minmax, running\_minmax &      68.110 &   68.230 &      68.030 &   68.292 \\
        \end{tabular}
        \caption{Results on ResNet18 for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    \end{subtable}

    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{l|rrrr}
        
         & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
         & Original BN & Reest BN & Original BN & Reest BN \\
        Range setting &             &          &             &          \\
        \hline
        MSE, MSE      &      69.448 &   \textbf{69.638} &       69.49 &   69.624 \\
        \end{tabular}
        \caption{Results on ResNet18 for fully flexible FP8 formats. Mantissa and exponent bits are set individually per quantizer, bias is set per channel. Best results are marked in bold.}
    \end{subtable}
    \caption{ResNet18 PTQ results}\label{tab:rn18full}
\end{table}

==> tables/salsanext_fp8_ptq_tables.tex <==
\begin{table}[h!]
    \begin{subtable}[]{\textwidth}
    % \begin{subfloat}[Results on SalsaNext for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.]
        \centering
        \begin{tabular}{ll|r}
        Mantissa bits & Bias & mIoU \\
        \hline
        5 & -1  & 21.521  \\
          &  1  & 22.238 \\
        4 &  4  & 55.788 \\
          &  3  & \textbf{55.792} \\
        3 &  8  & 54.918 \\
          &  9  & 54.914
        \end{tabular}
        \caption{Results on SalsaNext for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    % \end{subfloat}
    \end{subtable}
    
    
    \begin{subtable}[]{\textwidth}
    % \begin{subfloat}[Results on SalsaNext  esm  ,÷ for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.]
        \centering
        \begin{tabular}{ll|r}
         Mantissa bits & Range setting & MIoU \\
        \hline
        5 & MSE, MSE &      55.518  \\
        4 & MSE, MSE &      55.666  \\
        3 & MSE, MSE &      55.120  \\
        \end{tabular}
        \caption{Results on SalsaNext for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    % \end{subfloat}
    \end{subtable}
    \caption{SalsaNext PTQ results}\label{tab:salsanextfull}
\end{table}

==> tables/tasks_datasets_models.tex <==



\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
        Task & Dataset & Model(s) & Metric \\
        \hline
        \multirow{2}{*}{Classification} & \multirow{2}{*}{ImageNet} & ResNet18, MobileNetV2& \multirow{2}{*}{Top-1 Accuracy}\\
        && ViT\\
        Language understanding & GLUE & BERT-base & Macro-average\\
        Semantic Segmentation & Cityscapes & HRNet & mIoU \\
        Semantic Segmentation & Pascal VOC & DeepLabV3 (MobileNetV2) & mIoU \\
        LIDAR segmentation & SemanticKITTI & SalsaNext & mIoU\\
    \end{tabular}
    \caption{Tasks, datasets, and models used in our experiments.}
    \label{tab:tasks_datasets_models}
\end{table}

==> tables/vit_fp8_ptq_tables.tex <==
\begin{table}[h]

    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Bias &             &          &             &          \\
        \hline
        5 & -2  &       0.100 &    0.100 &       0.100 &    0.100 \\
          & -1  &       0.096 &    0.096 &       0.096 &    0.096 \\
          &  0  &       6.032 &    6.032 &       6.032 &    6.032 \\
          &  1  &      51.052 &   51.052 &      51.052 &   51.052 \\
        4 &  2  &      58.688 &   58.688 &      58.688 &   58.688 \\
          &  3  &      76.146 &   76.146 &      76.146 &   76.146 \\
          &  4  &      76.970 &   76.970 &      76.970 &   76.970 \\
          &  5  &      66.830 &   66.830 &      66.830 &   66.830 \\
        3 &  8  &      77.364 &   77.364 &      77.364 &   77.364 \\
          &  9  &      \textbf{77.366} &   \textbf{77.366} &      \textbf{77.366} &   \textbf{77.366} \\
          &  10 &      77.254 &   77.254 &      77.254 &   77.254 \\
          &  11 &      77.320 &   77.320 &      77.320 &   77.320 \\
        \end{tabular}
        \caption{Results on ViT for fixed FP8 formats. Formats are fixed for the full network. Best results are marked in bold.}
    \end{subtable}
    
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{ll|rrrr}
          &  & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
          &  & Original BN & Reest BN & Original BN & Reest BN \\
        Mantissa bits & Range setting &             &          &             &          \\
        \hline
        5 & MSE, MSE &      77.300 &   77.300 &      77.234 &   77.234 \\
          & current\_minmax, allminmax &      77.114 &   77.114 &      76.930 &   76.930 \\
          & current\_minmax, running\_minmax &      77.114 &   77.114 &      76.930 &   76.930 \\
        4 & MSE, MSE &      77.672 &   77.672 &      77.656 &   77.656 \\
          & current\_minmax, allminmax &      77.682 &   77.682 &      \textbf{77.706} &   \textbf{77.706} \\
          & current\_minmax, running\_minmax &      77.682 &   77.682 &      \textbf{77.706} &   \textbf{77.706} \\
        3 & MSE, MSE &      77.556 &   77.556 &      77.424 &   77.424 \\
          & current\_minmax, allminmax &      77.348 &   77.348 &      77.490 &   77.490 \\
          & current\_minmax, running\_minmax &      77.348 &   77.348 &      77.490 &   77.490 \\
        \end{tabular}
        \caption{Results on ViT for flexible bias FP8 formats. Mantissa and exponent bit widths are fixed per network, but each channel has its own bias value. Best results are marked in bold.}
    \end{subtable}
    
    \begin{subtable}[]{\textwidth}
        \centering
        \begin{tabular}{l|rrrr}
         & \multicolumn{2}{l}{Per channel} & \multicolumn{2}{l}{Per tensor} \\
         & Original BN & Reest BN & Original BN & Reest BN \\
        Range setting &             &          &             &          \\
        \hline
        MSE, MSE      &      77.614 &   77.614 &      \textbf{77.624} &   \textbf{77.624} \\
        \end{tabular}
        \caption{Results on ViT for fully flexible FP8 formats. Mantissa and exponent bits are set individually per quantizer, bias is set per channel. Best results are marked in bold.}
    \end{subtable}
    \caption{ViT PTQ results}\label{tab:vitfull}
\end{table}


